On Secure Workflow Decentralisation on the Internet

Decentralised workflow management systems are a new research area, where most work to-date has focused on the system's overall architecture. As little attention has been given to the security aspects in such systems, we follow a security driven approach, and consider, from the perspective of available security building blocks, how security can be implemented and what new opportunities are presented when empowering the decentralised environment with modern distributed security protocols. Our research is motivated by a more general question of how to combine the positive enablers that email exchange enjoys, with the general benefits of workflow systems, and more specifically with the benefits that can be introduced in a decentralised environment. This aims to equip email users with a set of tools to manage the semantics of a message exchange, contents, participants and their roles in the exchange in an environment that provides inherent assurances of security and privacy. This work is based on a survey of contemporary distributed security protocols, and considers how these protocols could be used in implementing a distributed workflow management system with decentralised control . We review a set of these protocols, focusing on the required message sequences in reviewing the protocols, and discuss how these security protocols provide the foundations for implementing core control-flow, data, and resource patterns in a distributed workflow environment.

==> eptcsdata.tex <==
\providecommand{\event}{Tom Van Cutsem and Mark S. Miller (Eds.):\\
Decentralized Coordination of Distributed Processes 2010}
\providecommand{\volume}{27}
\providecommand{\anno}{2010}
\providecommand{\firstpage}{2}
\providecommand{\eid}{2}
\pdfoutput=1

